DisCoCat for Donkey Sentences

We demonstrate how to parse Geach's Donkey sentences in a compositional distributional model of meaning. We build on previous work on the DisCoCat (Distributional Compositional Categorical) framework, including extensions that model discourse, determiners, and relative pronouns. We present a type-logical syntax for parsing donkey sentences, for which we define both relational and vector space semantics.

==> eptcsdata.tex <==
\providecommand{\firstpage}{32}
\providecommand{\publicationstatus}{M. Moortgat and M. Sadrzadeh (Eds.): Modalities in substructural logics.\\
Applications at the interfaces of logic, language and computation (AMSLO 2023).\\
EPTCS 381, 2023, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.381.5}{10.4204/EPTCS.381.5}}
\pdfoutput=1

